Tackling Dynamics in Federated Incremental Learning with Variational Embedding Rehearsal

Federated Learning is a fast growing area of ML where the training datasets are extremely distributed, all while dynamically changing over time. Models need to be trained on clients' devices without any guarantees for either homogeneity or stationarity of the local private data. The need for continual training has also risen, due to the ever-increasing production of in-task data. However, pursuing both directions at the same time is challenging, since client data privacy is a major constraint, especially for rehearsal methods. Herein, we propose a novel algorithm to address the incremental learning process in an FL scenario, based on realistic client enrollment scenarios where clients can drop in or out dynamically. We first propose using deep Variational Embeddings that secure the privacy of the client data. Second, we propose a server-side training method that enables a model to rehearse the previously learnt knowledge. Finally, we investigate the performance of federated incremental learning in dynamic client enrollment scenarios. The proposed method shows parity with offline training on domain-incremental learning, addressing challenges in both the dynamic enrollment of clients and the domain shifting of client data.

==> backup/architecture.tex <==

\subsection{Federated Incremental Learning}
\label{subsec:architecture}

\blue{\textbf{I think we can take this first paragraph and the figure and move it to Section 3.2 and remove this section altogether}}\\
Figure \ref{fig:block_diagram} describes the high-level structure of the proposed client- and server-side components. The goal of the proposed ``Federated Incremental Learning with Variational Embedding Rehearsal'' (FIL-VER) is: first to train a Variational Embedding Encoder (VEE) producing statistical, representations, federate the models and finally, rehearse on a subset of the client representations on the server, rather than replaying the raw data, i.e. the ``Naive Rehearsal'' approach~\cite{hsu2018re}. The proposed system consists of two main components: client-side representation extraction and training and server-side rehearsal. 
%
%\ddim{Following the FedAvg, Section~\ref{subsec:fedAvg}, it is hard to incorporate such a step in the FL setup, despite the fact that the Rehearsal process is important for Incremental Learning~\cite{hsu2018re}. The proposed system differs in the additional client-side processes: first, a probabilistic embedding encoder is initially trained, and then used as the front-end for the model training process. While local training is running, the learnt representations are sampled and sent to the server. All of current and previous representations (from the clients) are collected and used for server-side rehearsal.} 


\blue{\textbf{This is repeated later too}\\In this work two different approaches are investigated as part of the representation-based ``\textit{Federated Incremental Learning}'' (FIL): first, we investigate the deterministically extracted embedding-based FIL and then, VEE-based learning combined with Server-side Training (SST). The main difference between these scenarios is that in the first case, it is possible to reconstruct the clients' data, rendering any privacy constraints prohibitive. In the latter scenario, client raw data and representations are decoupled, and thus employed for the proposed FIL-VER system.}
%
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\textwidth]{pics/cst_and_sst.png}
    \caption{The concept of client-side training and SST. VER-Sampled case is our proposed method where client sends sampled VER vectors. On the other hand, VER-Stats is a framework we created for comparison where clients send to the server mean and variance values, which can infringe local privacy. }
    \label{fig:CST_SST}
    \vspace{-.2in}
\end{figure}


% \caption{Training and prediction mode of Variational Embedding Rehearsal (VER)  approach. In training mode: previously extracted (on clients) embeddings (from iterations $t\leq T-1$) are mixed with current data to train the model $\mathbf{w}^{(T)}$. In inference mode: The part of the encoder used to estimate the $\sigma^{(T)}$ is ignored, setting $\sigma^{(T)}=0$. The output of the encoder is used to generate training examples  $z^{(T)}$ for the Rehearsal step. \blue{We should replace right figure about inference and have TWO figures about VER-Samples and VER-Stats.}}
